Introduction of Multi-particle B\"{u}ttiker Probes -- Bridging the Gap between Drift Diffusion and Quantum Transport

State-of-the-art industrial semiconductor device modeling is based on highly efficient Drift-Diffusion (DD) models that include some quantum corrections for nanodevices. In contrast, latest academic quantum transport models are based on the non-equilibrium Green's function (NEGF) method that cover all coherent and incoherent quantum effects consistently. Carrier recombination and generation in optoelectronic nanodevices represent an immense numerical challenge when solved within NEGF. In this work, the numerically efficient B\"uttiker-probe model is expanded to include electron-hole recombination and generation in the NEGF framework. Benchmarks of the new multiple-particle B\"{u}ttiker probe method against state-of-the-art quantum-corrected DD models show quantitative agreements except in cases of pronounced tunneling and interference effects.

==> paper2_documentation.tex <==

\begin{itemize}

\item Presentation/Reports: 

2019 IWCN : \url{ https://nanohub.org/groups/klimeck/svn/trunk/StudentData/kuangchungwang/sphinx_log/source/Documentation/IWCN2019.pptx}

2018 NUSOD: \url{https://nanohub.org/groups/klimeck/svn/trunk/StudentData/kuangchungwang/sphinx_log/source/Documentation/2018nusod.pptx}

2018 SISPAD: \url{https://nanohub.org/groups/klimeck/svn/trunk/StudentData/kuangchungwang/sphinx_log/source/Documentation/2018_sispad_slide.pptx}

\item Fig.\ref{eta_mobility}

 	Folder:  \url{https://nanohub.org/groups/klimeck/svn/trunk/StudentData/kuangchungwang/sphinx_log/source/201711_buttikerprobe/4_flat_band_mobility}
 	
 	figure: \path{eta_mobility.png}
 	
 	raw data for the plot : 
 	\\\path{eta_mobility_1e20input_refine_bandedge_uniform_fixedK_flat_contacteta.in}
 	\\\path{eta_mobility_1e20input_refine_bandedge_uniform_fixedK_hole_flat_contacteta.in}
 	
 	inputs templates(requires the script to change parameters):
 	\\\path{input_refine_bandedge_uniform_fixedK_hole_flat_contacteta.in }
 	\\\path{input_refine_bandedge_uniform_fixedK_flat_contacteta.in}
 	
 	Script to produce all inputdecks ramping different parameters e.g.  voltages doping: 
 	\\\verb|./submit_voltage.sh sub 0 1e20 input_refine_bandedge_uniform_fixedK_flat_contacteta.in|
 	\\\verb|./submit_voltage.sh sub 0 1e20 input_refine_bandedge_uniform_fixedK_hole_flat_contacteta.in|
 	
 	
 	
\item Fig.\ref{pn_charge}
  
  DD raw datafolder: 	
  \\\url{ https://nanohub.org/groups/klimeck/svn/trunk/StudentData/kuangchungwang/sphinx_log/source/201711_buttikerprobe/silvaco_DD_comparison/pn_junction_updatedparam_update_mobi/well_Vd3.000000e+00_doping1e20pn1.in_jac_9_emesh_32_kmesh_20_kmax_0.5}
  
  DD input: \url{https://nanohub.org/groups/klimeck/svn/trunk/StudentData/kuangchungwang/sphinx_log/source/201711_buttikerprobe/silvaco_DD_comparison/pn_junction_updatedparam_update_mobi/pn1.in }
  
  NEGF raw data folder:  
  \\\url{https://nanohub.org/groups/klimeck/svn/trunk/StudentData/kuangchungwang/sphinx_log/source/201711_buttikerprobe/3_e_h_coupled_resonance_expdecay_semiclassical_GaN_EcEv_sym_exp_withpoisson_contacteta/Vd3.000000e+00_doping1e20input_refine_bandedge_uniform_fixedK_etaleads_urback.in_jac_9_emesh_128_kmesh_40_kmax_0.1_oneshot_}
  
  Contour raw data: 
  \\\path{bprgf_e_backward_solver_device_energy_resolved_k_integrated_density.dat}
  \\\path{bprgf_h_backward_solver_device_energy_resolved_k_integrated_density.dat}
  \\spatial density data:  \path{debug_n.dat} \path{debug_p.dat}
 	
  input deck :
  \\\url{https://nanohub.org/groups/klimeck/svn/trunk/StudentData/kuangchungwang/sphinx_log/source/201711_buttikerprobe/3_e_h_coupled_resonance_expdecay_semiclassical_GaN_EcEv_sym_exp_withpoisson_contacteta/Vd3.000000e+00_doping1e20input_refine_bandedge_uniform_fixedK_etaleads_urback.in_jac_9_emesh_128_kmesh_40_kmax_0.1_oneshot_/temp_3.000000e+00_1e20input_refine_bandedge_uniform_fixedK_etaleads_urback.in_jac_9_emesh_128_kmesh_40_kmax_0.1.in}

\item Fig.\ref{pn_recomb}

 	DD data for 3.0V:     \url{https://nanohub.org/groups/klimeck/svn/trunk/StudentData/kuangchungwang/sphinx_log/source/201711_buttikerprobe/silvaco_DD_comparison/pn_junction_updatedparam_update_mobi/well_Vd3.000000e+00_doping1e20pn1.in_jac_9_emesh_32_kmesh_20_kmax_0.5} 
 	
 	DD data for 3.6V \url{https://nanohub.org/groups/klimeck/svn/trunk/StudentData/kuangchungwang/sphinx_log/source/201711_buttikerprobe/silvaco_DD_comparison/pn_junction_updatedparam_update_mobi/well_Vd3.600000e+00_doping1e20pn1.in_jac_9_emesh_32_kmesh_20_kmax_0.5} 
 	
 	Band profile:  \verb|Ec.dat  Ev.dat|
    
    spatially resolved recombination:   \verb| A.dat  B.dat  C.dat|	

 	
 	NEGF data for 3.0V:  
 	\\input \url{https://nanohub.org/groups/klimeck/svn/trunk/StudentData/kuangchungwang/sphinx_log/source/201711_buttikerprobe/3_e_h_coupled_resonance_expdecay_semiclassical_GaN_EcEv_sym_exp_withpoisson_contacteta/temp_3.000000e+00_1e20input_refine_bandedge_uniform_fixedK_etaleads_urback.in_jac_9_emesh_128_kmesh_40_kmax_0.1.in}
 	 \\folder \url{https://nanohub.org/groups/klimeck/svn/trunk/StudentData/kuangchungwang/sphinx_log/source/201711_buttikerprobe/3_e_h_coupled_resonance_expdecay_semiclassical_GaN_EcEv_sym_exp_withpoisson_contacteta/Vd3.000000e+00_doping1e20input_refine_bandedge_uniform_fixedK_etaleads_urback.in_jac_9_emesh_128_kmesh_40_kmax_0.1trial_0}
 	
 	NEGF data for 3.6V: 
 	\\input \url{https://nanohub.org/groups/klimeck/svn/trunk/StudentData/kuangchungwang/sphinx_log/source/201711_buttikerprobe/3_e_h_coupled_resonance_expdecay_semiclassical_GaN_EcEv_sym_exp_withpoisson_contacteta/Vd3.600000e+00_doping1e20input_refine_bandedge_uniform_fixedK_etaleads_urback.in_jac_9_emesh_128_kmesh_40_kmax_0.1trial_0}
 	\\folder \url{https://nanohub.org/groups/klimeck/svn/trunk/StudentData/kuangchungwang/sphinx_log/source/201711_buttikerprobe/3_e_h_coupled_resonance_expdecay_semiclassical_GaN_EcEv_sym_exp_withpoisson_contacteta/temp_3.600000e+00_1e20input_refine_bandedge_uniform_fixedK_etaleads_urback.in_jac_9_emesh_128_kmesh_40_kmax_0.1.in}
 	
 	
 	
 	
\item Fig.\ref{pn_IV}
 	
 	DD Folder: \url{https://nanohub.org/groups/klimeck/svn/trunk/StudentData/kuangchungwang/sphinx_log/source/201711_buttikerprobe/silvaco_DD_comparison/pn_junction_updatedparam_update_mobi/}
 	DD IV raw data : \path{IVtotal_1e20pn1.in}  \path{total_re}
 	
 	NEGF data folder: \url{https://nanohub.org/groups/klimeck/svn/trunk/StudentData/kuangchungwang/sphinx_log/source/201711_buttikerprobe/3_e_h_coupled_resonance_expdecay_semiclassical_GaN_EcEv_sym_exp_withpoisson_contacteta}
 	
 	NEGF IV  data: \path{wellIVtotal_1e20input_refine_bandedge_uniform_fixedK_well_etaleads.in} \path{wellIVrecomb_1e20input_refine_bandedge_uniform_fixedK_well_etaleads.in}
 	
    NEGF job script:   \path{./overlord.sh}	
  
 	Simulation Results: 
    \\poisson calculation output : \path{Vd*_doping1e20input_refine_bandedge_uniform_fixedK_well_etaleads_urbach.in_jac_9_emesh_128_kmesh_40_kmax_0.1trial_0}
 	\\current conservation loop output : \path{Vd*_doping1e20input_refine_bandedge_uniform_fixedK_well_etaleads_urbach.in_jac_9_emesh_128_kmesh_40_kmax_0.1_oneshot_}
 
   
    
\item Fig.\ref{qw_band_charge}

 	DD data Folder: 
 	\url{https://nanohub.org/groups/klimeck/svn/trunk/StudentData/kuangchungwang/sphinx_log/source/201711_buttikerprobe/silvaco_DD_comparison/pn_junction_well_capture_escape_with_radiative_SRH_Auger_for_bound_states_with_pn_update_mobi/well_Vd2.600000e+00_doping1e20optimizeEkmesh_jac_9_emesh_32_kmesh_20_kmax_0.5}
 	\\Figure: \path{np_xnm_log2.png }   \path{Ec.png} \path{Ev.png}
 	\\input: \path{../qw1.in}

 	NEGF data Folder: 
 	\url{https://nanohub.org/groups/klimeck/svn/trunk/StudentData/kuangchungwang/sphinx_log/source/201711_buttikerprobe/3_e_h_coupled_resonance_expdecay_semiclassical_GaN_EcEv_sym_exp_withpoisson_contacteta/Vd2.600000e+00_doping1e20input_refine_bandedge_uniform_fixedK_well_etaleads_urbach.in_jac_9_emesh_128_kmesh_40_kmax_0.1_oneshot_}
 	\\input: \path{temp_2.600000e+00_1e20input_refine_bandedge_uniform_fixedK_well_etaleads_urbach.in_jac_9_emesh_128_kmesh_40_kmax_0.1.in}
 	\\Contour raw data: 
 	\\\path{bprgf_e_backward_solver_device_energy_resolved_k_integrated_dos.dat}
 	\\\path{bprgf_h_backward_solver_device_energy_resolved_k_integrated_dos.dat}
 	\\density data:  \path{debug_n.dat} \path{debug_p.dat}
\item Fig.\ref{qw_occu}
	
	 DD File : 
 	\\\url{https://nanohub.org/groups/klimeck/svn/trunk/StudentData/kuangchungwang/sphinx_log/source/201711_buttikerprobe/silvaco_DD_comparison/pn_junction_well_capture_escape_with_radiative_SRH_Auger_for_bound_states_with_pn_update_mobi/well_Vd4.000000e+00_doping1e20optimizeEkmesh_jac_9_emesh_32_kmesh_20_kmax_0.5}
 	\\ Band profile: \path{Ec.dat} \path{Ev.dat} 
 	
 	NEGF File:
 	\\folder: \url{https://nanohub.org/groups/klimeck/svn/trunk/StudentData/kuangchungwang/sphinx_log/source/201711_buttikerprobe/3_e_h_coupled_resonance_expdecay_semiclassical_GaN_EcEv_sym_exp_withpoisson_contacteta/Vd4.000000e+00_doping1e20input_refine_bandedge_uniform_fixedK_well_etaleads_urbach.in_jac_9_emesh_128_kmesh_40_kmax_0.1_oneshot_}
 	\\contour data: 
 	 \\\path{bprgf_e_backward_solver_device_energy_resolved_k_integrated_density.dat}
 	 \\\path{bprgf_h_backward_solver_device_energy_resolved_k_integrated_density.dat}
\item Fig.\ref{qw_IV}
 	  
 	  Figure file:
 	  \\\url{https://nanohub.org/groups/klimeck/svn/trunk/StudentData/kuangchungwang/sphinx_log/source/201711_buttikerprobe/silvaco_DD_comparison/pn_junction_well_capture_escape_with_radiative_SRH_Auger_for_bound_states_with_pn_update_mobi/IVlog_eta0.05_comp.png}
 	  \\\url{https://nanohub.org/groups/klimeck/svn/trunk/StudentData/kuangchungwang/sphinx_log/source/201711_buttikerprobe/silvaco_DD_comparison/pn_junction_well_capture_escape_with_radiative_SRH_Auger_for_bound_states_with_pn_update_mobi/IV_eta0.05_comp.png}
 	
 	NEGF data folder: \\\url{https://nanohub.org/groups/klimeck/svn/trunk/StudentData/kuangchungwang/sphinx_log/source/201711_buttikerprobe/3_e_h_coupled_resonance_expdecay_semiclassical_GaN_EcEv_sym_exp_withpoisson_contacteta}

    processing commands is in \path{./overlord.sh}
    
 	IV raw data : 
 	 \\\path{wellIVtotal_1e20input_refine_bandedge_uniform_fixedK_well_etaleads.in}
 	 \\\path{wellIVrecomb_1e20input_refine_bandedge_uniform_fixedK_well_etaleads.in}
 	
 	raw data files: 
 	\path{Vd*_doping1e20input_refine_bandedge_uniform_fixedK_well_etaleads_urbach.in_jac_9_emesh_128_kmesh_40_kmax_0.1_oneshot_}
    \path{Vd*_doping1e20input_refine_bandedge_uniform_fixedK_well_etaleads_urbach.in_jac_9_emesh_128_kmesh_40_kmax_0.1trial_0}
    
 	DD data folder: 
 	\\\url{https://nanohub.org/groups/klimeck/svn/trunk/StudentData/kuangchungwang/sphinx_log/source/201711_buttikerprobe/silvaco_DD_comparison/pn_junction_well_capture_escape_with_radiative_SRH_Auger_for_bound_states_with_pn_update_mobi/}
 	
\item Fig.\ref{qw_solar}

 	NEGF folder :
 	\\\url{https://nanohub.org/groups/klimeck/svn/trunk/StudentData/kuangchungwang/sphinx_log/source/201711_buttikerprobe/3_e_h_coupled_resonance_expdecay_semiclassical_GaN_EcEv_sym_exp_withpoisson_solar_contacteta}
 	
 	input template: 
 	\\\path{input_refine_bandedge_uniform_fixedK_well_contacteta_100k.in}
 	\\\path{input_refine_bandedge_uniform_fixedK_well_contacteta.in}
 	
 	script: \path{overlord.sh} 
 	
 	figure:\path{IVnew350k_100knew.png}
 	
 	raw data: 
 	\path{IV_350K IVsolar_half_350k IVsolar_350k IVsolar_100k ,well_new_IVtotal_1e20input_refine_bandedge_uniform_fixedK_well_contacteta.in_gen0 ,well_new_IVtotal_1e20input_refine_bandedge_uniform_fixedK_well_contacteta.in_gen1.325E-18, well_new_IVtotal_1e20input_refine_bandedge_uniform_fixedK_well_contacteta.in_gen2.65E-18, well_new_IVtotal_1e20input_refine_bandedge_uniform_fixedK_well_contacteta_100k.in_gen2.65E-18}
 	
 	DD folder :
 	\url{https://nanohub.org/groups/klimeck/svn/trunk/StudentData/kuangchungwang/sphinx_log/source/201711_buttikerprobe/silvaco_DD_comparison/pn_junction_well_capture_escape_with_radiative_SRH_Auger_for_bound_states_with_pn_update_mobi_solarcell/photogeneration_after_fix/}
 	\\input decks: \path{well_temp_2.600000e+00_1e20optimizeEkmesh_jac_9_emesh_32_kmesh_20_kmax_0.5_m.in
,well_temp_2.600000e+00_1e20optimizeEkmesh_jac_9_emesh_32_kmesh_20_kmax_0.5_m_solar.5.in
,well_temp_2.600000e+00_1e20optimizeEkmesh_jac_9_emesh_32_kmesh_20_kmax_0.5_m_solar.in
,well_temp_2.600000e+00_1e20optimizeEkmesh_jac_9_emesh_32_kmesh_20_kmax_0.5_m_solar_100k.in}

\end{itemize}
